Towards Fine-Grained Reasoning for Fake News Detection

The detection of fake news often requires sophisticated reasoning skills, such as logically combining information by considering word-level subtle clues. In this paper, we move towards fine-grained reasoning for fake news detection by better reflecting the logical processes of human thinking and enabling the modeling of subtle clues. In particular, we propose a fine-grained reasoning framework by following the human information-processing model, introduce a mutual-reinforcement-based method for incorporating human knowledge about which evidence is more important, and design a prior-aware bi-channel kernel graph network to model subtle differences between pieces of evidence. Extensive experiments show that our model outperforms the state-of-the-art methods and demonstrate the explainability of our approach.

==> src/notation.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notation table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Notation}

\issue{REMOVE THIS OR PUT THIS IN THE SUPPLEMENT BEFORE SUBMISSION}

\indent Modules are highlighted in \textbf{textbf}, such as \textbf{Textual-based Reasoning Channel}

Theorems and concepts are highlighted in \textit{textit}, such as $\textit{Mutual Reinforcement}$

Sets are denoted with capital letters, such as $P$ for the set of posts and $P_r$ for the set of posts that are related to topic $T_r$. Similarly, $T$ is the set of topics. $t_r$ is the $r$-th topic

Representations are in mathrm. For example, $\mathbf{t}_r$ is the topic representation of $T_r$.

Individual nodes are denoted with lowercase letters, such as $p_i$ for the $i$-th post

$\omega_{u_i, u_j}$: edge weight between two users (same for post / keywords)

$C_{i}$: retweets regarding $p_i$. This notation is used ONLY once, so I am considering replacing it with something like "$\textrm{ret(i)}$"


$N_P, N_K, N_U$: number of posts, keywords, and users in $G$

$N_T$: number of topics

$M$: number of training examples

$W_P, W_K, W_U$: weight matrices for posts, keywords, and users

$\mathbb{P}(Y\mid X)$: Bayesian probability. 

The mathbb-style notation is taken from: % https://en.wikipedia.org/wiki/Notation_in_probability_and_statistics





$E_P$: prior saliency of the set of posts $P$

$\varphi(t_{r})$: evidence ranking features

$\delta(G)$: graph-based evidence fusion representation

${L}_{q, r}$ is the translation matrix between $q$ and $r$ in textual-based reasoning channel. $\tilde{L}_{q, r}$ is its equivalence in social-based reasoning channel.
